CEmb-SAM: Segment Anything Model with Condition Embedding for Joint Learning from Heterogeneous Datasets

Automated segmentation of ultrasound images can assist medical experts with diagnostic and therapeutic procedures. Although using the common modality of ultrasound, one typically needs separate datasets in order to segment, for example, different anatomical structures or lesions with different levels of malignancy. In this paper, we consider the problem of jointly learning from heterogeneous datasets so that the model can improve generalization abilities by leveraging the inherent variability among datasets. We merge the heterogeneous datasets into one dataset and refer to each component dataset as a subgroup. We propose to train a single segmentation model so that the model can adapt to each sub-group. For robust segmentation, we leverage recently proposed Segment Anything model (SAM) in order to incorporate sub-group information into the model. We propose SAM with Condition Embedding block (CEmb-SAM) which encodes sub-group conditions and combines them with image embeddings from SAM. The conditional embedding block effectively adapts SAM to each image sub-group by incorporating dataset properties through learnable parameters for normalization. Experiments show that CEmb-SAM outperforms the baseline methods on ultrasound image segmentation for peripheral nerves and breast cancer. The experiments highlight the effectiveness of Cemb-SAM in learning from heterogeneous datasets in medical image segmentation tasks.

==> images/fig1.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.85\linewidth]{images/Fig 1 Method (13).png}
\end{center}
\vspace{-5mm}
\caption{ (A) CEmb-SAM: \textit{Segment Anything model} with Condition Embedding block. Input images come from heterogeneous datasets, i.e., peroneal and ulnar nerve dataset, and the model is jointly trained to segment both types of nerves. The sub-group condition is fed into Condition Embedding block and encoded into sub-group representations. Then, image embeddings are combined with sub-group representations. In the figure, different regions, peroneal and ulnar, are segmented, respectively. We fixed image and prompt encoder while fine-tuning Condition Embedding block and mask decoder. (B) Detailed description of Condition Embedding Block. The sub-group condition is encoded into condition representation parameters $\gamma$ and $\beta$. The input feature $\textnormal{F}^{\tiny \textnormal{in}}$ is scaled and shifted using sub-group representation parameters.}
\label{fig:fig1}
\end{figure*}
